A Multi-level procedure for enhancing accuracy of machine learning algorithms

We propose a multi-level method to increase the accuracy of machine learning algorithms for approximating observables in scientific computing, particularly those that arise in systems modeled by differential equations. The algorithm relies on judiciously combining a large number of computationally cheap training data on coarse resolutions with a few expensive training samples on fine grid resolutions. Theoretical arguments for lowering the generalization error, based on reducing the variance of the underlying maps, are provided and numerical evidence, indicating significant gains over underlying single-level machine learning algorithms, are presented. Moreover, we also apply the multi-level algorithm in the context of forward uncertainty quantification and observe a considerable speed-up over competing algorithms.

==> Old/algorithm.tex <==
\section{The multilevel machine learning algorithm}


==> Old/code.tex <==
\section{Obtaining the code}
\todo{Roberto: Describe where they can download the code for the experimetn (github url, then we can upload it to some permanent url later)}
https://github.com/mroberto166/ThesisProject/tree/development

Writing the readme file

==> Old/conclusions.tex <==
\section{Conclusions}



==> Old/experiments.tex <==
\section{Numerical experiments}
\label{sec:6}
In this section, we present two numerical examples in order to asses   the predictive performance of the multilevel model, in particular with respect to the classical single level model.  In this context,  a sensitivity study is conducted in order to provide a guideline for the design of the multilevel model. Moreover, within the framework of Uncertainty Quantification, we compare the performance of machine learning algorithms, and in particular the multilevel algorithm, with the statistical sampling Quasi Monte Carlo and Multilevel Quasi Monte Carlo methods. 


\subsection{Projectile Motion}
\label{sec:ProjMot}
To begin with, let us consider the simple example of a projectile motion with an additional drag force term, described by the following Cauchy problem:
\begin{eqnarray}
\label{parab_syst}
\left\{
\begin{aligned}
\frac{d}{dt}\boldsymbol{x}(t;y) &= \boldsymbol{v}(t;y) 
\\[5pt]
\frac{d}{dt}\boldsymbol{v}(t; y) &= - {{F}_D\big(\boldsymbol{v}(t;y); y \big)}\boldsymbol{e}_1 - g\boldsymbol{e}_2
\\[5pt]
\boldsymbol{x}(y;0)&= \boldsymbol{x}_0(y)
\\[5pt]
\frac{d\boldsymbol{x}(y;0)}{dt} &= \boldsymbol{v}_0(y)
\end{aligned}
\right.
\end{eqnarray}
Here, ${F}_D = \frac{1}{2m}\rho C_d {\pi r^2}|| \boldsymbol{v}||^2$ denotes the drag force
and $\boldsymbol{x}_0(y) = [0, ~h]$, $\boldsymbol{v}_0(y) = [v_0\cos(\alpha), ~v_0\sin(\alpha)]$ are the initial position and velocity of the object. 
We set
\begin{equation}
\begin{aligned}
\rho(y)=1.225\big(1 + \varepsilon G_1(y)\big),\quad 
r(y)&=0.23\big(1 + \varepsilon G_2(y)\big),\quad 
C_D(y)=0.1\big(1 + \varepsilon G_3(y)\big)
\\\
m(y)=0.145\big(1 + \varepsilon G_4(y)\big),\quad 
h(y)&=\big(1 + \varepsilon G_5(y)\big),\quad
\alpha(y)=30^\circ\big(1 + \varepsilon G_6(y)\big)
\\\
v_0(y)&=25\big(1 + \varepsilon G_7(y)\big)
\end{aligned}
\end{equation}
where $\varepsilon=0.1$ is the perturbation term, $y \in [0,1]^7$ and $G_k(y)= 2y_k -1$ for $k=1,...,7.$
The observable for this problem is chosen as the  \textit{horizontal range} $x_{max}$, 
\begin{equation}
	\map(y) = x_{max}(y) = x_1(y;t_f),\quad \text{with}~~ t_f = x_2^{-1}(0) 
\end{equation}

\subsection{Convergence Analysis of Generalization Error}
In the first place, we want to numerically investigate the error bound \eqref{eq:genE2}. As we pointed in Remark \ref{re:sharpness}, the bound is not necessarily sharp, and therefore, we aim at computing the so-called \textit{compression}, namely the amount by which we overestimate the generalization error.  To this end, we consider the problem setting described above and employ neural network model ${\map}^\ast(y)$ to approximate the parameter to the observable map $\map(y)$.
We choose the following set of hyperparameters for the neural network:
\begin{itemize}
	\item 6 hidden layers ;
	\item 10 neurons per layer;
	\item \textit{Mean Absolute Error} loss function ($p=1$ in \eqref{eq:lf1});
	\item ADAM optimizer with learning rate $\eta = 0.01$;
	\item $L^2$ regularization with $\lambda= 10^{-6}$
\end{itemize}
According to the hypotheses of Theorem \ref{theo:1}, we assume that the training set
\begin{equation}
	\train =  \Big\{\Big(y_i, \map(y_i)\Big),~ 1\leq i \leq M\Big\}
\end{equation}
is  \textit{independently} and \textit{identically} drawn from the \textit{uniform} distribution $\mu(y)$. The observable $\map(y_i)$ is computed by solving \eqref{parab_syst} with $\Delta t = 0.00125$. 

We train a neural network in the form of \eqref{eq:ann1} with different values of the samples size $N=16,~32,~64,~128,~256,~512,~1024$ and compute the generalization and training errors for each of them. The generalization error is estimated by computing \eqref{eq:egen} on a testing set of dimension $N_\test=$ 1968, 1936, 1872, 1744, 1488, 976. As we stated in Theorem \ref{theo:1}, the bound has to be interpreted in the \textit{root mean square} sense. Therefore, for each value of $N$, we retrain the neural network $K=60$ times and compute the mean square error of the generalization and training error, together with the bound \eqref{eq:genE2}. In this regard, the terms $std{({\map}^\ast)}$, is computed by evaluating the corresponding network ${\map^\ast}$ with $N_{ML}=1000$ uniformly distributed samples and computing the standard deviation of the model outputs. The compression rate is estimated by dividing the values claimed by the bound and the values obtained by the the numerical computation of $\er_G$. 

The results of the convergence analysis are reported in \figurename{ \ref{fig:conv}}. On one hand, \figurename{ \ref{fig:bounds}} shows that the training error $\er_{T}$ is, in general, rather low and assumes almost constant value. The generalization error, on the other, reduces at constant rate equal to 0.82, slightly faster that the rate predicted by the theoretical estimate. Nevertheless, the bound appears quite accurate, in particular if compared with existing bounds, with a compression between 2 and 6, that is rather satisfactory.

\begin{figure}[!t]
	\begin{subfigure}{.49\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{{Images/bounds}}
		\caption{}
		\label{fig:bounds}
	\end{subfigure}
	\begin{subfigure}{.49\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{{Images/compression}}
		\caption{}
		\label{fig:compression}
	\end{subfigure}
	\caption{Convergence analysis of generalization error \ref{fig:bounds} and corresponding compression \ref{fig:compression} with respect to the theoretical estimate.  }
	\label{fig:conv}
\end{figure}



\subsubsection{Predictive Performance of the Multilevel Model and Sensitivity Study to Design Parameters} 
For this problem we consider a total number of 7 consecutive resolutions $s_G=\{0,...,L\}$ with $L=6$.  The dataset at the resolution $L=6$ accounts for 2000 samples, generated for testing purpose. The input samples $y_i$ are drawn from a uniform measure $\mu(y)$. We use the time step $\Delta t_0 = 0.08$ for the solution of (\ref{parab_syst}) at the coarsest resolution $\ell=0$. Moreover, we uniquely employ neural network to learn the parameters to the observable map (i.e. $\alpha_{NN}=1$ and $\alpha_{GP}=0$ in the ensemble model definition).

The ensemble of configurations employed for the sensitivity analysis consists of 4 different sequences of resolutions, drawn from $s_G$:
\begin{equation}
\begin{aligned}
s^1_n =& \{0, ~6\},\quad &c_{ml} = &0.16
\\
s^2_n =& \{0, ~3, ~6\},\quad &c_{ml} =& 0.67
\\
s^3_n =& \{0, ~2, ~4, ~6\},\quad &c_{ml} =& 1.5
\\
s^4_n =& \{0, ~1, ~2, ~3, ~4,~5, ~6\},\quad &c_{ml} =& 6.0
\end{aligned}
\end{equation}
and the following values for the number of training samples at the coarsest and finest resolution levels:
\begin{equation}
N_0 =\{256, ~512,~ 1024, ~2048\},
\end{equation}
\begin{equation}
N_L =\{4, ~8, ~16, ~32, ~64, ~92, ~128\}.
\end{equation}
This set of parameters generates an ensemble of 112 different multilevel models whose performances with respect to the single level model are assessed as discussed in Section \ref{sec:sens}. The testing set accounts for all the high fidelity dataset samples not included in the training process. Therefore, its size varies between 1872 and 1996 samples. 
The results of the ensemble training for the hyperparameters selection and  sensitivity study are presented below. 

\vspace{3mm}
\textbf{Results of the Ensemble Training.}  The ensemble training is performed as discussed in Section \ref{ch:implementation}. We employ $512$ samples in order to tune the hyperparameters of the neural network model ${\map}^\ast_{0,NN}$ and $256$ for the specification of the  model $\dtl^\ast_{ref, NN}$. We fix the same reference architecture for both ${\map}^\ast_{0, NN}$ and $\dtl^\ast_{ref, NN}$, consisting of 6 layers and 10 neurons per layer. The best performing configuration of hyperparameters turns out to be the same for both the maps, corresponding to $L^2$ regularization with $\lambda=5\cdot10^{-7}$. 
\begin{figure}[!h]
	\centering
	\begin{subfigure}{.48\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_tot_x_max}}
		\caption{Relative mean prediction error versus computational cost of the competing models}
		\label{fig:mpe_time_tot_x_max}
	\end{subfigure}
	\begin{subfigure}{.48\linewidth}
		\includegraphics[width=1\textwidth]{{Images/error_cost_x_max}}
		\caption{Average speed up of the multilevel model with respect to the standard scheme versus computational cost}
		\label{fig:error_cost_x_max}
	\end{subfigure}
	\caption{Overall performance of the multilevel model compared to standard scheme for Projectile Motion example.}
	\label{fig:overall_parab}
\end{figure}
\begin{figure}[!h]
	\centering
	\begin{subfigure}{.48\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_tot_x_max_sob}}
		\caption{Relative mean prediction error versus computational cost of the competing models (with uniformly distributed points and neural network model)}
		\label{fig:mpe_time_tot_x_max_sob}
	\end{subfigure}
	\begin{subfigure}{.48\linewidth}
		\includegraphics[width=1\textwidth]{{Images/error_cost_x_max_sob}}
		\caption{Average speed up of the multilevel model with respect to the standard scheme versus computational cost (with low-discrepancy Sobol points and ensemble model)}
		\label{fig:error_cost_x_max_sob}
	\end{subfigure}
	\caption{Overall performance of the multilevel model compared to standard scheme for Projectile Motion example.}
	\label{fig:overall_parab_sob}
\end{figure}

\vspace{3mm}
\textbf{Overall Performance of the Multilevel Model compared to the Standard Model.} 
Overall, the multilevel model outperforms the classical scheme, with increase in efficiency up to 12 times for few model configurations (\figurename{ \ref{fig:error_cost_x_max}}). Almost all the multilevel configurations (95\%) result in better predictive performance compared to single level model and  7\% ensures a speed up of one order of magnitude, that is quite encouraging (\figurename{ \ref{fig:overall_parab}}). Moreover, the multilevel model appears more efficient than the competing single level scheme for all the ranges of computational cost, although in the range of large computational cost the speed up drop up to 2.



\vspace{3mm}
\textbf{Sensitivity Study Results.} 
 A more detailed insight of the problem can be inferred from the sensitivity analysis of the multilevel model performances to the design parameters. 
 \begin{itemize}
     \item \textit{Choice of the number of samples at the coarsest level $N_0$}. \figurename{ \ref{fig:mpe_time_x_max_0}} shows that increasing the number of samples at the coarsest resolution results, at large extent, in better accuracy of the model. However, this does not hold true for the models corresponding to range where $\er_G<1\%$, since it merely results in a rise of the computational cost of the model. This behavior can be explained by the fact that such configurations correspond to rather small number of training samples at the finest resolution ($N_L=$ 4 or 8) and the sequence of resolutions accounting for only two levels $s_n=\{0,L\}$. Under these circumstances, the assumption $std(\map^\Delta_0)\gg std(\dtl_1)$ is violated and the accuracy of the model is dominated by the poor approximation of the detail that annihilates the advantages of enlarging the number of samples $N_0$.
     \item  \textit{Choice of the model complexity $c_{ml}$}. The sensitivity of the model efficiency to the model complexity is depicted in \figurename{ \ref{fig:mpe_time_x_max_1}}. The plot shows that intermediate complexities $c_{ml}=0.67$ and $c_{ml}=1.5$ definitely lead to a better efficiency of the model, particularly in the regione where $\er_G<1\%$. 
     \item  \textit{Choice of the number of samples at the finest level $N_L$}. \figurename{ \ref{fig:mpe_time_x_max_2}} reveals indeed the strong influence of the number of training samples on the computational cost of the model, as mentioned before. Therefore, the choice on the number of samples $N_L$ is mostly dictated by the resources available to address a given problem. However, for this problem it does not seem to strongly impinge on the efficiency speed up. In fact, thanks to the great flexibility of the multilevel scheme, for any choice of the parameter $N_L$, proper configurations of the remaining parameters can be chosen to achieve the desired accuracy.
 \end{itemize}
 

 

 
\vspace{3mm}
\subsubsection{Uncertainty Quantification Results}
In order to asses the performance of multilevel machine learning algorithm in UQ, a numerical reference solution is computed using $M=20000$ samples and time-step $\Delta t = 0.001$. \figurename{ \ref{fig:uq_parab}} depicts the mean squared error for the estimation of the mean, standard deviation and probability distribution (in terms of the Wasserstein distance) versus the computational cost of competing algorithms. For the single level model we adopt the models trained by using $N_L^{sl} = 9,~15,~21,~64,~191,~322$ high-fidelity samples. The selection of the multilevel model design configurations is dictated by the sensitivity study performed above. We choose some of the best performing ones (Table \ref{tab:parab_MLmlearn}). 

Overall, both the learning schemes perform more efficiently compared to the statistical sampling methods, resulting in much more accurate approximation of the observable statistics for a significant  range of the computational cost. Moreover, even higher accuracy can be achieved by increasing the number of samples $J_L$ employed to feed the trained model, clear evidence of the advantages of using machine learning in the framework of uncertainty quantification. Also, the high efficiency of the multilevel scheme also translates into a relevant speed up compared to the classical single level model. In particular, the multilevel machine learning model results approximately 5, 4 and 3 times more efficient than Quasi Monte Carlo, multilevel Quasi Monte Carlo and classical machine learning scheme (Table \ref{tab:sum_parab_UQ}) for the approximation of the probability distribution, with peaks up to 8, 6, and 8.
\begin{table}[!h] 
	\centering 
	\footnotesize{
		\begin{tabular}{c c |  c |  c|  c | c } 
			\toprule
			\bfseries  &\multicolumn{5}{c}{\bfseries MLML Configurations}\\
			\midrule
			\bfseries Samples $N_0$  & 256 & 256 & 2048 & 2048 & 2048\\[3pt]
			\bfseries Samples $N_L$ & 4 & 8 & 8 & 32 & 64\\[3pt]
			
			\bfseries Complexity $c_{ml}$ & 0.17 & 0.67 & 0.67 & 0.67 & 1.5 \\[3pt]
			
			\bottomrule 
		\end{tabular}
	}
		\caption{Different cost configurations used to evaluate the performance of multilevel machine learning method  for the Projectile Motion example.}
		\label{tab:parab_MLmlearn}
\end{table}
\begin{table}[!h] \centering
	\footnotesize
	\begin{tabular}{c c c c c c c c c}\toprule
		& 
		\multicolumn{2}{c}{\bfseries QMC} 
		&\phantom{abc}& 
		\multicolumn{2}{c}{\bfseries MLQMC} 
		&\phantom{abc}& 
		\multicolumn{2}{c}{\bfseries SLML}\\
		\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
		& Mean & Max && Mean& Max && Mean & Max \\ \midrule
		
\bfseries Mean & 4.8&10.9 && 4.1&7.7 && 2.7 &12.1 \\
\bfseries Dev & 5.8&8.6 && 3.5&6.2 && 5.9 &14.5 \\
\bfseries Dist & 4.8&7.8 && 3.9&6.0 && 2.9 &7.9 \\


		\bottomrule
	\end{tabular}
	\caption{Average and maximum speed up of multilevel machine learning scheme compared to competing models for the estimation of mean, standard deviation and probability distribution for the Projectile Motion example over the entire range of computational costs.}
	\label{tab:sum_parab_UQ}
\end{table}




\subsection{Flow past RAE2822 airfoil}

\begin{comment}
\begin{figure}[!h]
	\centering
	
		\includegraphics[width=0.6\linewidth]{{Images/airf}}
	\caption{RAE2822 airfoil shape: $\bar{S}_u(x)$ and $\bar{S}_l(x)$, $x\in[0,1]$, are the upper and lower surface, respectively.}
	\label{fig:airf_shape}
\end{figure}
\end{comment}



We consider the example of non-viscous, compressible flow past an RAE2822 airfoil, treated by Lye, Mishra and Ray \cite{lye2019deep}. 
%The airfoil is depicted in \figurename{ \ref{fig:airf_shape}}. $\bar{S}_u(x)$ and $\bar{S}_l(x)$ denote the upper and lower surface of the airfoil, respectively. 
The problem is described by the two-dimensional Euler equations \cite{fvm} augmented with suitable initial and boundary conditions. We consider the following perturbed free stream conditions and the profile geometry:
\begin{equation}
\begin{aligned}
T^\infty(y)&= \big(1 + \varepsilon_1 G_1(y)\big),\quad 
M^\infty(y)=0.729\big(1 + \varepsilon_1 G_2(y)\big), 
\\[5pt]
p^\infty(y)&= \big(1 + \varepsilon_1 G_2(y)\big),\quad
\alpha(y)=2.31^\circ\big(1 + \varepsilon_1 G_6(y)\big)
\\[5pt]
S_L(x;y)&= \overline{S}_L(x)\big(1 + \varepsilon_2 G_4(y)\big),\quad 
S_U(x;y)=\overline{S}_U(x)\big(1 + \varepsilon_2 G_4(y)\big),
\end{aligned}
\end{equation}
where $\alpha$ is the angle of attack and $\bar{S}_U(x)$, $\bar{S}_L(x)$, $x\in[0,1]$, denote the unperturbed upper and lower surfaces of the airfoil, respectively. $G_k$ are defined as in the previous numerical examples and $\varepsilon_1=0.1$, $\varepsilon_2=0.2$. 
The observables are the lift and drag coefficients:
\begin{equation}
\map_1(y) =
C_L(y) = \frac{1}{E_k^\infty(y)}\int_{S_L\cup S_U}p(y)n(y)\cdot\hat{y}(y)ds,\quad
\end{equation}
\begin{equation}
\map_2(y) =
C_D(y) = \frac{1}{E_k^\infty(y)}\int_{S_L\cup S_U}p(y)n(y)\cdot\hat{x}(y)ds,\quad
\end{equation}
where $\hat{x}(y) = [\cos(\alpha(y)), \sin(\alpha(y))]$, $\hat{y}(y) = [-\sin(\alpha(y)), \cos(\alpha(y))]$ and
\begin{equation}
	E_k^\infty(y)= \frac{\rho^\infty(y)||\textbf{u}^\infty(y)||^2}{2},
\end{equation}
is the free-stream kinetic energy. 

\subsubsection{Predictive Performance of the Multilevel Model and Sensitivity Study to Design Parameters} 
For this problem, a total number of 5 resolution levels $\ell=0,...,L$ with $L=4$ are considered. In line with the previous example, we generate a total number 2000 samples at resolution $L=4$ to test the results of our multilevel model. According to the results obtained by Lye, Mishra an Ray \cite{lye2019deep} for this problem, we employ low-discrepancy Sobol points to generate the training sets, as they have proven exceptional performance  compared to uniformly distributed random points.

In order to perform the sensitivity study we choose four different sequences of mesh resolutions with different model complexities:
\begin{equation}
\begin{aligned}
\label{eq:conf_seq_airf}
s^1_n =& \{0, ~4\},\quad &c_{ml} = &0.25
\\
s^2_n =& \{0, ~2, ~4\},\quad &c_{ml} =& 1.0
\\
s^3_n =& \{0, ~2, ~3, ~4\},\quad &c_{ml} =& 2.31
\\
s^4_n =& \{0, ~1, ~2, ~3, ~4\},\quad &c_{ml} =& 4.0
\end{aligned}
\end{equation}
and the same ensemble of configurations for the training samples at the coarsest and finest mesh resolutions as in the previous numerical example. 

\vspace{3mm}
\textbf{Results of the Ensemble Training.} For the lift coefficient we proceed similarly to the previous case study.
%: we use the \textit{same} hyperparameters configuration for \textit{each} detail ${\dtl}^\ast_{\ell_k}$, $1\leq k\leq n$, defined by the ensemble training performed on the difference function $\er_{ref}^{cv} = {C}_L^{(1)} - {C}_L^{(0)}$.  
As far as neural network model is concerned, we exploit the results achieved by Lye, Mishra and Ray \cite{lye2019deep} also for the selection of the network architecture, accounting for 9 hidden layers with 12 units. Optimizer, learning rate and loss function are chosen as usual ({ADAM, $\eta=0.01$ and mean squared loss function}). This reference initial setting has been employed for both the surrogates $\map^\ast_{0,NN}$ and  $\dtl_{ref,NN}$. Starting from this reference setting, two distinct ensemble trainings have been performed, one for the selection of the hyperparameters of the model $\map^\ast_{0,NN}$ using 512 samples and one for the detail $\dtl_{ref,NN}$ using 256 samples. Also for the lift coefficient, the best performing configuration is the same for both the maps and accounts for $L^2$ regularization and $\lambda=5\cdot 10^{-7}$.
\begin{table}[!t] 
	\centering
	\renewcommand{\arraystretch}{1.1} 
	
	\footnotesize{
		\begin{tabular}{c c c c c c c c } 
			\toprule
			\bfseries   &\bfseries Samples &\bfseries Val. Size & \bfseries Lear. Rate &\bfseries $L^1$ - Reg. & \bfseries $L^2$ - Reg. &\bfseries Width &\bfseries Height \\ 
			\midrule
			\midrule
			$\map^{\Delta_0}$            & 1024  & 15\% & 0.001 &0& $5\cdot10^{-7}$& 6& 16\\
			\midrule 
			$\map^{\Delta_1} - \map^{\Delta_0}$ & 256 &  15\% & 0.001 &0& $10^{-6}$& 6& 12\\
				\midrule 
			$\map^{\Delta_2} - \map^{\Delta_1}$ & 64 &15\% & 0.001 &$5\cdot10^{-7}$& 0& 6& 12\\
				\midrule 
			$\map^{\Delta_3} - \map^{\Delta_2}$ & 64 & 15\% &0.01 &$5\cdot10^{-6}$& 0& 6& 8\\
				\midrule 
			$\map^{\Delta_4} - \map^{\Delta_3}$ & 8 & 15\% &0.01 &$10^{-5}$& 0& 6& 8\\
				\midrule 
			$\map^{\Delta_2} - \map^{\Delta_0}$ & 256 & 15\% & 0.001 &$5\cdot10^{-7}$& 0& 6& 8\\
			\midrule
			$\map^{\Delta_4} - \map^{\Delta_2}$ & 8 &  15\% &0.01 &$5\cdot10^{-7}$& 0& 6& 12\\
				\midrule 
			$\map^{\Delta_3} - \map^{\Delta_0}$ & 256 &15\% & 0.001 &$5\cdot10^{-7}$& 0& 9& 16\\
			\midrule 
			$\map^{\Delta_4} - \map^{\Delta_0}$ & 32 & 15\% &0.001 &$10^{-5}$& 0& 6& 8\\
			\bottomrule
		\end{tabular}
	\caption{Best performing \textit{Neural Network} configurations for the drag coefficient}
		\label{setting_drag_net}
	}
\end{table}

For the Gaussian Process we perform the ensemble training employing 256 samples for the selection of the covariance function of $\map^\ast_{0,GP}$ and 128 for the reference detail $\dtl^\ast_{ref,GP}$. Matern kernel with $\nu=1.5$ results in the best performance of the Gaussian process regressor for both the maps.

For the drag coefficient, on the other hand, we perform a massive ensemble training choosing the best set of hyperparameters for each model complexity listed in (\ref{eq:conf_seq_airf}) and for each term in the definition of the corresponding multilevel model (\ref{eq:def_mlml_gen}). Moreover, the ensemble training includes not only the selection of the exponent $q$ of the regularization term and the regularization parameter $\lambda$, but also the learning rate and the network architecture as well. ADAM optimizer and mean squared error are employed as in the rest of this work. The number of layer is chosen among four different values: 8, 12, 16, 20, 24. For the number of neurons, on the other hand, we use the values 8, 12, 16, 20, 24. Three values of the learning rate are chosen: $\eta=$0.001, 0.005 and 0.01. The candidates of the regularization parameter $\lambda$ and exponent of the regularization term $q$ are the same as in the remaining examples. The best performing configurations for each map of interest are reported in Table \ref{setting_drag_net}.

For the Gaussian process, the same model configuration used for the lift coefficient has proven to perform accurately also for the drag and for all the difference maps. 
\begin{figure}[!h]
	\begin{subfigure}{\textwidth}
		\centering
		\includegraphics[width=0.49\linewidth]{{Images/mpe_time_tot_Lift}}
		\includegraphics[width=0.49\linewidth]{{Images/mpe_time_tot_Drag}}
		\caption{Relative mean prediction error versus computational cost of the competing models}
		\label{fig:mpe_time_tot_airf}
	\end{subfigure}
		\begin{subfigure}{\textwidth}
		\centering
		\includegraphics[width=0.49\linewidth]{{Images/error_cost_Lift}}
		\includegraphics[width=0.49\linewidth]{{Images/error_cost_Drag}}
		\caption{Average speed up of the multilevel model with respect to the standard scheme versus computational cost}
		\label{fig:error_cost_airf}
	\end{subfigure}
	\caption{Overall performance of the multilevel model compared to standard scheme for the lift (on the left) and drag coefficient (on the right).}
	\label{fig:overall_airf}
\end{figure}

\vspace{3mm}
\textbf{Overall Performance of the Multilevel Model compared to the Standard Model.} 
Also for this example, we observe that, for both the aerodynamic coefficients, the majority of the multilevel model configurations performs more efficiently than the corresponding standard machine learning model, representing approximately the 70-75\% of the entire ensemble of configurations, although the accuracy speed is lower if compared to the Projectile Motion example (\figurename{ \ref{fig:mpe_time_tot_airf}}). Moreover, a small fraction of parameter settings (3\% for the lift and 8\% for the drag) results into a 4 time reduction of the prediction error compared to the single level models. Similarly to the previous numerical example, we observe a monotonous decrease of the average accuracy speed up as we consider progressively larger computational costs (\figurename{ \ref{fig:error_cost_airf}}). In particular for very high costs the speed up is around one, suggesting that both the models perform equally well. However, we would like to point out that in real applications one usually does not have access to a such amount of resources, and in the real range of applicability, the multilevel model turns out to be more efficient than the classical model.

\vspace{3mm}
\textbf{Sensitivity Study Results.} 
\begin{itemize}
    \item \textit{Choice of the number of samples at the coarsest level $N_0$}. The variation of the model efficiency with respect to the number of training samples at the coarsest grid is depicted in Figures \ref{fig:mpe_time_Lift_0}, \ref{fig:mpe_time_Drag_0}. In line with the results of the projectile motion, for both the aerodynamic coefficients the most efficient multilevel models are the ones trained by using a large number of samples at the coarsest resolution. 
    %However, in the range of very low computational cost, the configurations corresponding to $N_0>500$ are penalized comparing to $N_0=256$ according to the same arguments discussed above. 
    \item \textit{Choice of the model complexity $c_{ml}$}. The sensitivity of the model efficiency to the model complexity is plotted in Figures \ref{fig:mpe_time_Lift_1}, \ref{fig:mpe_time_Drag_1}. For this problem as well, intermediate model complexities, in particular $c_{m}=1$, appear to improve the efficiency of the multilevel. We argue that the enhanced results obtained with the intermediate complexities are explained by the fact that they provide a good balance between the accuracy and cost of the model, compared to the others that are either too expensive or inaccurate.
    \item \textit{Choice of the number of samples at the finest level $N_L$}. Figures \ref{fig:mpe_time_Lift_2}, \ref{fig:mpe_time_Drag_2} show that  the number of training sampling $N_L$ heavily impinges on  the computational cost of the model, similarly to previous example. In particular, as we increase the number of samples the multilevel model speed up reduces, consistently with the plots in Figure \ref{fig:error_cost_airf}, and with obvious implications on the accuracy of the model. Therefore, a large number of training samples $N_L$ is usually preferable as it results in lower prediction errors, although under these circumstance, both the models are valuable choices in light of the low speed up.
    %Reasonably, this also results into better accuracy of the models. In fact, a large number of training samples at the finest grid translates into larger number of samples across each layer of the model, and lower prediction error in turn.  
    %Moreover, here the number of samples $N_L$ seems to have a much stronger impact on the overall performance of the multilevel model compared to the single level one because the complexity of the problem translates into slightly worse approximation of the building pieces of the model. In fact, the prediction error achieved with both the model are one order of magnitude larger than the projectile motion example.
\end{itemize}



\subsubsection{Uncertainty Quantification Results}
The reference solution is computed by using $M=2000$ samples on the mesh resolution $L=4$. For the single level algorithm we employ the models trained by using $N_L^{sl} = 4,~7,~16,~32,~64,~128,~144,~228,~256$ samples for the lift coefficient and $N_L^{sl} = 4,~8,~16,~32,~110,~128$ for drag. 
We report in Tables \ref{tab:lift_MLmlearn}, \ref{tab:drag_MLmlearn} the design parameters of the multilevel models employed in the comparison. 


\begin{table}[!h] 
	\centering 
	\footnotesize
		\begin{tabular}{c c |  c |  c|  c | c | c |c | c |c|c} 
			\toprule
			\bfseries  &\multicolumn{10}{c}{\bfseries MLML Configurations}\\
			\midrule
			\bfseries Samples $N_0$  & 512 & 1024 & 2048 & 256 & 2048& 2048 &2048& 2048 &2048&2048 \\[3pt]
			\bfseries Samples $N_L$ & 4 & 4 & 4 & 4 & 4& 8 &32 &64& 92 &92 \\[3pt]
			\bfseries Complexity $c_{ml}$ & 0.25 & 0.25 & 0.25 & 1 & 1 & 1& 1 &4 &1 &2.31 \\[3pt]
			\bottomrule 
		\end{tabular}
\caption{Different cost configurations used to evaluate the performance of multilevel machine learning model for the lift statistics approximation.}
\label{tab:lift_MLmlearn}
\end{table}
\begin{table}[!h] 
	\centering 
	\footnotesize
	\begin{tabular}{c c |  c |  c|  c | c | c |c } 
	\toprule
	\bfseries  &\multicolumn{7}{c}{\bfseries MLML Configurations}\\
	\midrule
	\bfseries Samples $N_0$  & 256 & 512 & 512 & 512 & 1024& 1024 & 2048   \\[3pt]
	\bfseries Samples $N_L$ & 4 & 4 & 4 & 8 & 64& 64 & 92  \\[3pt]
	\bfseries Complexity $c_{ml}$ & 0.25 & 0.25 & 1 & 5 & 1 & 1 & 1 \\[3pt]
	\bottomrule 
\end{tabular}
\caption{Different cost configurations used to evaluate the performance of multilevel machine learning model for the drag  statistics approximation.}
	\label{tab:drag_MLmlearn}
\end{table}
The  resulting plots \textit{relative error versus computational time}  are show in Figures \ref{fig:uq_lift}, \ref{fig:uq_drag} for the lift and drag coefficients, respectively. Also for the airfoil example, the multilevel model reveals to be the most efficient scheme to capture the statistics of the observable. For instance, for the lift coefficient it results on average 9, 5 and 2 times more efficient in approximating the observable distribution, compared to Quasi Monte Carlo, Multilevel Quasi Monte Carlo and single level machine learning model, respectively (Table \ref{tab:sum_airf_UQ}). Similar results have been achieved for the drag with an average speed up of 5, 3.5 and 2 with respect to the competing schemes. 

\begin{table}[!h] \centering
	\footnotesize
	\begin{tabular}{c | c c c c c c c c c}\toprule
		\multicolumn{2}{c}{\bfseries }&
		\multicolumn{2}{c}{\bfseries QMC} 
		&\phantom{abc}& 
		\multicolumn{2}{c}{\bfseries MLQMC} 
		&\phantom{abc}& 
		\multicolumn{2}{c}{\bfseries SLML}\\
		\cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10}
	 	\multicolumn{2}{c}{\bfseries }&Mean & Max && Mean& Max && Mean & Max \\ \midrule
		 \multirow{ 3}{*}{{\bfseries Lift}}
		    &\bfseries Mean & 12.4&19.6 && 3.5&12.8 && 1.0 &1.4 \\
            &\bfseries Dev & 5.9&16.9 && 4.1&23.3 && 4.1 &68.5 \\
            &\bfseries Dist & 9.2&11.4 && 5.4&6.4 && 1.7 &4.0 \\
		 \midrule
		 \multirow{ 3}{*}{{\bfseries Drag}}%\input{UQ_sp_Drag.txt}
    		 &\bfseries Mean & 12.8&18.4 && 5.7&9.4 && 1.7 &6.8 \\
            &\bfseries Dev & 5.5&9.9 && 3.3&5.3 && 3.0 &5.3 \\
            &\bfseries Dist & 4.8&6.8 && 3.5&5.2 && 1.8 &3.8 \\

		 
		\bottomrule
	\end{tabular}
	\caption{Average and maximum speed up of multilevel scheme compared to competing models for the estimation of mean, standard deviation and probability distribution for the aerodynamic coefficients.}
		\label{tab:sum_airf_UQ}
\end{table}


\begin{figure}[!h]
	\centering
	\begin{subfigure}{.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_x_max_1}}
		\caption{Sensitivity to $N_0$}
		\label{fig:mpe_time_x_max_0}
	\end{subfigure}
	\begin{subfigure}{.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_x_max_2}}
		\caption{Sensitivity to $c_{ml}$}
		\label{fig:mpe_time_x_max_1}
	\end{subfigure}
	\begin{subfigure}{0.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_x_max_0}}
		\caption{Sensitivity to $N_L$}
		\label{fig:mpe_time_x_max_2}
	\end{subfigure}
	\caption{Results of the sensitivity analysis of the multilevel model performance to the design parameters for the \textit{Projectile Motion} numerical example (uniformly distributed random points and neural network model).}
	\label{fig:mpe_time_parab}
\end{figure}
\begin{figure}[!h]
	\centering
	\begin{subfigure}{.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_x_max_1_sob}}
		\caption{Sensitivity to $N_0$}
		\label{fig:mpe_time_x_max_0_sob}
	\end{subfigure}
	\begin{subfigure}{.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_x_max_2_sob}}
		\caption{Sensitivity to $c_{ml}$}
		\label{fig:mpe_time_x_max_1_sob}
	\end{subfigure}
	\begin{subfigure}{0.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_x_max_0_sob}}
		\caption{Sensitivity to $N_L$}
		\label{fig:mpe_time_x_max_2_sob}
	\end{subfigure}
	\caption{Results of the sensitivity analysis of the multilevel model performance to the design parameters for the \textit{Projectile Motion} numerical example (low-discrepancy Sobol points and ensemble model).}
	\label{fig:mpe_time_parab_sob}
\end{figure}
\begin{figure}[!h]
	\centering
	\begin{subfigure}{.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_Lift_1}}
		\caption{Sensitivity to $N_0$}
		\label{fig:mpe_time_Lift_0}
	\end{subfigure}
	\begin{subfigure}{.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_Lift_2}}
		\caption{Sensitivity to $c_{ml}$}
		\label{fig:mpe_time_Lift_1}
	\end{subfigure}
	\begin{subfigure}{0.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_Lift_0}}
		\caption{Sensitivity to $N_L$}
		\label{fig:mpe_time_Lift_2}
	\end{subfigure}
	\caption{Results of the sensitivity analysis of the multilevel model performance to the design parameters for the lift coefficient of \textit{RAE2822 Airfoil} numerical example.}
	\label{fig:mpe_time_Lift}
\end{figure}
\begin{figure}[!h]
	\centering
	\begin{subfigure}{.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_Drag_1}}
		\caption{Sensitivity to $N_0$}
		\label{fig:mpe_time_Drag_0}
	\end{subfigure}
	\begin{subfigure}{.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_Drag_2}}
		\caption{Sensitivity to $c_{ml}$}
		\label{fig:mpe_time_Drag_1}
	\end{subfigure}
	\begin{subfigure}{0.325\linewidth}
		\includegraphics[width=1\textwidth]{{Images/mpe_time_Drag_0}}
		\caption{Sensitivity to $N_L$}
		\label{fig:mpe_time_Drag_2}
	\end{subfigure}
	\caption{Results of the sensitivity analysis of the multilevel model performance to the design parameters for the drag coefficient of \textit{RAE2822 Airfoil} numerical example.}
	\label{fig:mpe_time_parab}
\end{figure}


\begin{figure}[!t]
	\centering
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_x_max_mean}}
		\caption{Estimation of the mean}
		\label{fig:x_max_mean}
	\end{subfigure}
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_x_max_std}}
		\caption{Estimation of the standard deviation}
		\label{fig:x_max_std}
	\end{subfigure}
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_x_max_wass}}
		\caption{Estimation of the PDF}
		\label{fig:x_max_wass}
	\end{subfigure}
	\caption{
	Relative mean squared error versus computational costs of competing models for the estimation of the horizontal range statistics.   Uniformly distributed random points and neural network models are used in the training process.
	}
	\label{fig:uq_parab}
\end{figure}
\begin{figure}[!t]
	\centering
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_x_max_mean_sob}}
		\caption{Estimation of the mean}
		\label{fig:x_max_mean_sob}
	\end{subfigure}
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_x_max_std_sob}}
		\caption{Estimation of the standard deviation}
		\label{fig:x_max_std_sob}
	\end{subfigure}
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_x_max_wass_sob}}
		\caption{Estimation of the PDF}
		\label{fig:x_max_wass_sob}
	\end{subfigure}
	\caption{
	Relative mean squared error versus computational costs of competing models for the estimation of the horizontal range statistics. Sobol points and ensemble models are used in the training process.
	}
	\label{fig:uq_parab_sob}
\end{figure}
\begin{figure}[!t]
	\centering
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_Lift_mean}}
		\caption{Estimation of the mean}
		\label{fig:x_max_mean}
	\end{subfigure}
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_Lift_std}}
		\caption{Estimation of the standard deviation}
		\label{fig:x_max_std}
	\end{subfigure}
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_Lift_wass}}
		\caption{Estimation of the PDF}
		\label{fig:x_max_wass}
	\end{subfigure}
	\caption{
	Relative mean squared error versus computational costs of competing models for the estimation of the lift coefficient statistics.
	}
	\label{fig:uq_lift}
\end{figure}
\begin{figure}[!t]
	\centering
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_Drag_mean}}
		\caption{Estimation of the mean}
		\label{fig:x_max_mean}
	\end{subfigure}
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_Drag_std}}
		\caption{Estimation of the standard deviation}
		\label{fig:x_max_std}
	\end{subfigure}
	\begin{subfigure}{.325\textwidth}
		\includegraphics[width=1\linewidth]{{Images/UQ_Drag_wass}}
		\caption{Estimation of the PDF}
		\label{fig:x_max_wass}
	\end{subfigure}
	\caption{
	Relative mean squared error versus computational costs of competing models for the estimation of the drag coefficient statistics.
	}
	\label{fig:uq_drag}
\end{figure}


==> Old/extensions.tex <==
\section{Extensions and Implementation}
\label{sec:5}

\subsection{Quasi-Monte Carlo type algorithms}


\begin{comment}


\subsection{Generalization of Multilevel Machine Learning Formulation}

The formulation of the multilevel scheme can be generalized considering a generic sequence of \textit{successive}, instead of \textit{consecutive}, mesh resolutions $s_n = \{\ell_n\}_{k=0}^{n}$, with $\ell_0=0$ and $\ell_n=L$, such that:
\begin{equation}
	\Delta_k = \Delta_L  2^{(\ell_n -\ell_k)} ~ 0 \leq k \leq n..
\end{equation}
Therefore, (\ref{eq:tsum}) can be rearranged accordingly:
\begin{equation}
\label{eq:def_mlml_gen}
\map^{\Delta_L}(y) = \map^{\Delta_0}(y) + \sum\limits_{k=1}^n \left(\underbrace{\map^{\Delta_{\ell_k}}(y) - \map^{\Delta_{\ell_{k-1}}}(y)}_{:=\dtl_{k}(y)}\right), \quad \forall y \in Y.
\end{equation}
The objective of the multilevel model turns now to learning the maps:
\begin{equation}
    \label{eq:ml1_gen}
    \map^{\Delta_0} (y) \approx \map_0^{\ast} (y), \quad \dtl_{k} (y) \approx \dtl^{\ast}_{k}(y), \quad \forall y\in Y, ~ 1 \leq k \leq n.
\end{equation}    
According to the generalization of the multilevel model, we introduce the \textit{model complexity} defined as:
\begin{equation}
	c_{ml} = \frac{n^2}{L},\quad \frac{1}{L}\leq c\leq L.
\end{equation}
For the simplest sequence of resolution, $s_0 =\{0, L\}$, we have $n=1$ and  $c=\frac{1}{L}$, whereas for the most complex sequence, defined by consecutive levels $s_n = \{0,1,...,L-1, L\}$, $n=L$ and the model complexity results $c_{ml}=L$. 


Based on the estimate (\ref{eq:genEml3}), we expect that, as long as $std(\dtl_k)\ll std(\map^{\Delta_0})$, the main contribution to the generalization error is given by the approximation of $\map^{\Delta_0}$, dependent on the number of training samples $N_0$.  Moreover, as we hinted before, the cost required to solve the underlying PDE (\ref{eq:ppde}) at the resolution $\Delta_k$ scales as $\Delta_k^{-(d_s+1)}$. Therefore, the number of samples $N_L$ generated at the resolution $\Delta_L$ will mostly contribute to the total cost of the model, being $\Delta_{\ell_n}<\Delta_{\ell_{n-1}}<\ldots<\Delta_{\ell_{0}}$. The obvious conclusion of these observations is that, together with the model complexity, we can control the efficiency on the model by carefully choosing $N_L$ and $N_0$ and, thus, denote $N_0$, $N_L$ and $c_{ml}$ as \textit{design parameters} of the multilevel model.

In practice, we choose the number of points used to train the intermediate details $\dtl_{k}$ as:
\begin{equation}
\label{points_int}
N_k = N_L2^{e(\ell_n-\ell_k)},\quad 0< k < n
\end{equation}
with
\begin{equation}
e = \frac{\log_2(N_0/N_L)}{L}.
\end{equation}



\end{comment}





\subsection{Other surrogate models}
\subsubsection{Gaussian Process Regressions}
{Gaussian Process} belongs to the class of methods known with the name of Bayesian models, founded on the homonymous Bayes' theorem \cite{}.
%The idea behind a Bayesian model is to assume that the map $\map$ is drawn from a function distribution  defined \textit{a priori} (\textit{prior}) and correct our belief on the nature of $\map$ with the knowledge of the experimental data distribution (\textit{likelhood}), in order to obtain the most probable distribution (\textit{posterior}) describing the function underlying the set of observations.

To define a Gaussian process we adopt the \textit{function-space view} described by \cite{GP}.
In this perspective, a {Gaussian Process} is shortly define as a Gaussian distribution over the functions $\map(y)$.
In the spirit of Gaussian Process model, we assume that the underlying function $\map(y)$ is drawn from a Gaussian Process with mean function $m({{y}})=\E{\map({y})}$ and covariance function $	k({{y}}, {y}')=\E{(\map({y}) - m({y})) (\map({y}') - m({y}'))}$ :
\begin{equation}
\map({y}) \sim GP(m({y}), k({y}, {y}')).
\end{equation}
or, in vector notation
\begin{equation}
\pazocal{L}\sim \mathcal{N}\big({\mu}, G\big),
\end{equation}
where ${\mu}_i = m(y_i)$ and $G$ is the Gram matrix, defined as:
\begin{equation}
G^{(i,j)} = k(\text{y}_{i}, \text{y}_{j}),
\end{equation}
for some vector of input samples $\{\text{y}_i\}$.
The choice of the mean and covariance function is totally arbitrarily and expresses our \textit{a priori} belief about the structure of the function before observations become available. 
It is customary to assume that $m({y}) = 0$. 

Let us now assume that the function $\map$ is known for some \textit{training samples} $ \{ ({{y}}_{i},z_{i}) ~|~ i=1,...,n\}$ and that the observations are noisy-free:
\begin{equation}
	\text{z}_i = \map(y_i).
\end{equation} 
This is not true in general, but in the case of data stemming from computer simulations it is legit to assume that the data are noisy-free, or characterized by noise with negligible variance \cite{design_exper}.
We are interested in embedding the information on the training set, or the \textit{likelihood} of the data, to our \textit{a priori} assumption on the function $\map$. To this end, we consider a set of test inputs $\text{y}_{\ast, j}$, $j = 1,...,n_*$ and  define the joint probability distribution of the training and test outputs ($\text{z}$ and $\text{z}_*$) as:
\begin{equation}
\begin{bmatrix}
\text{z}  \\[0.3em]
\text{z}_*  
\end{bmatrix} \sim \mathcal{N}\Bigg(\text{0}, \begin{bmatrix}
G & G_*  \\[0.3em]
G_*^T & G_{**}  
\end{bmatrix}\Bigg).
\end{equation}
Here, $G\in\mathbb{R}^{n\times n}$, $G_{*}\in\mathbb{R}^{n\times n_*}$ and $G_{**}\in\mathbb{R}^{n_*\times n_*}$ are the training, the training-test and test Gram matrices, respectively: 
\begin{equation}
G^{(i,j)} = k(\text{y}_{i}, \text{y}_{j}),\quad G_{*}^{(i,j)} = k(\text{y}_{i}, \text{y}_{*,j}),\quad\text{and}\quad G_{**}^{(i,j)} = k(\text{y}_{*,i}, \text{y}_{*,j}).
\end{equation}
The conditional probability $p(\text{z}_*|\text{y}_*, Y, \text{z})$ can be readily obtained, being $\text{z}$ and $\text{z}_*$  jointly \textit{Gaussian} random vectors:
\begin{equation}
	p(\text{z}_*|\text{y}_*, y, \text{z}) = \mathcal{N}\big(~G_*^T G^{-1}\text{z},~~ G_{**} - G_*^TG^{-1}G_*~\big).
\end{equation}
The computation of the conditional probability $p(\text{z}_*|\text{y}_*, Y, \text{z})$ demands the inversion of the training Gram matrix, usually performed with Cholesky algorithm. The cost of inverting the Gram matrix is $\mathcal{O}(n^3)$, where $n$ is the number of training samples. Therefore, the cost of Gaussian Process models grows rather fast as the number of training samples increases and this limits the range of applicability to problems with small size of datasets. However, this does not represent an obstacle in computational science, since the  size of the data obtained from simulations is usually small.

Popular choices for the covariance function are the squared exponential (also know with the name of RBF function) and Matern covariance function 
\begin{equation}
\label{eq:SE_cov}
	k_{SE}({y}, {y}') = \exp{\bigg(-\frac{|| {y} - {y}'||^2}{2\ell^2}\bigg)}
\end{equation}
\begin{equation}
\label{eq:mat_cov}
	 k_{Matern}(y, y')={\frac {2^{1-\nu }}{\Gamma (\nu )}}{\Bigg (}{\sqrt {2\nu }}{\frac {||y -y'||}{\ell }}{\Bigg )}^{\nu }K_{\nu }{\Bigg (}{\sqrt {2\nu }}{\frac {||y -y'||}{\ell }}{\Bigg )},
\end{equation}
where $||\cdot||$ denotes the standard euclidean norm, $K_\nu$ is the Bessel function [ref] and $\ell$ the \textit{characteristic length}, describing the length scale of the mutual influence between the points $\text{y}$ and $\text{y}'$. The Matern kernel assumes simple shape when the coefficient $\nu$ is half-integer.


\subsubsection{Ensemble Models}
One common technique used in machine learning is the \textit{model averaging}, consisting in the design of a new model by assembling together different models trained separately from one another. 
The resulting model, denoted as \textit{ensemble model}, is proven to perform better than the single ones \cite{goodfellow}. 

Let us consider a set of $L$ different regression models. Let $y_{{ensemble}}$ be the prediction given by the ensemble model on a test set, defined by:
\begin{equation}
\label{eq:ens_def}
	y_{ensemble} = \frac{1}{L}\sum_l y_l,
\end{equation}
where $y_l$ denotes, on the other hand, the prediction provided by the model $l$. Moreover, let $e_l$ be the error committed by the model $l$ on a single sample of the test set and $e_{{ensemble}}$ the ensemble prediction error:
\begin{equation}
	e_{\text{ensemble}} = \frac{1}{L}\sum_{l=1}^{L}e_l.
\end{equation}
The expected mean squared error of the ensemble predictor over the entire test set is 
\begin{equation}
	\bbE{\bigg( \frac{1}{L}\sum_{l}e_l \bigg)^2}= \frac{1}{L^2}\bbE{\bigg( \sum_{l}e_l^2 + \sum_{m\neq l} e_me_l \bigg)^2} = \frac{1}{L}v + \frac{L-1}{L}c
\end{equation}
where we have defined $\E{e_l^2}=v$, and $\E{e_le_m}=c$, $\forall l,m$. If the models errors are uncorrelated ($c=0$), we have that 
\begin{equation}
\bbE{\bigg( \frac{1}{L}\sum_{l}e_l \bigg)^2}=  \frac{1}{L}v,
\end{equation}
suggesting that the mean squared errors decreases linearly with the total number of regressors employed. However, in practice, this holds true if the performance of all the models are comparable to each other. If this is not the case, one could reasonable expect that the performance of the ensemble model results worse than the best performing one. We observe that (\ref{eq:ens_def}) is a linear combination of the model prediction, where all the models are given the same weight, equal to $\frac{1}{L}$. Therefore, to enhance the predictive performance of the ensemble model we can rewrite the linear combination in a more general form:
\begin{equation}
\label{eq:general_ens_def}
y_{ensemble} = \sum_l \alpha_l y_l.
\end{equation}
The coefficient of the linear combination can be obtained by simple linear regression, using a set of data point not belonging to the training set. In this way, each model is given a different weight based on its own performance, resulting overall into better performance, regardless of the performance of the single models. 
\subsection{Extended Algorithm to Design a Multilevel Machine Learning Model}
Equipped with the extensions presented above, we provide the algorithm for the training of a more general variant of the multilevel model,  employed in the next numerical examples below.

\begin{algorithm} 
\label{alg:ext_ML} {\bf Multi-level learning of parameters to observable map}. 
\begin{itemize}
\item [{\bf Inputs}:] Parameterized PDE \eqref{eq:ppde}, Observable \eqref{eq:obsp}, high-resolution numerical method for solving \eqref{eq:ppde} and calculating \eqref{eq:obsp}, sequence of mesh resolutions $s_n$, number of training samples $N_0$, number of training samples $N_L$.
\item [{\bf Goal}:] Find a machine learning model $\map^{\ast}_{ml}$ for approximating the parameters to observable map $\map$ \eqref{eq:ptoob}. 

\item [{\bf Step $1$}:] For the coarsest mesh resolution $\ell_0$, select a training set $\train_0 = \{y^0_i\},~1 \leq i \leq N_0 = \#(\train_0)$. For each $y^0_i$, compute $\map^{\Delta}_0(y^0_i)$ by solving the PDE \eqref{eq:ppde} on a mesh resolution $\Delta_0$ and computing the observable \eqref{eq:obsp}.  With the training data $\{y^0_i,\map^{\Delta_0}(y^0_i)\}_{1 \leq i \leq N_0}$, train the neural network $\map^{\ast}_{0,NN} \approx \map^{\Delta}_0$ and the Gaussian Process regressor $\map^{\ast}_{0,NN} \approx \map^{\Delta}_0$, with suitable choice of the model hyperparameters. Assemble the ensemble model $\map^{\ast}_{0} = \alpha_{NN}\map^{\ast}_{0,NN} + \alpha_{GP}\map^{\ast}_{0,GP}$

\item [{\bf Step $2$}:] For each $\ell_k \in s_n$, $1 \leq k \leq n$, select a training set $\train_k = \{y^{\ell_k}_i\},~1 \leq i \leq N_k = \#(\train_k)$, with $N_k$ defined as in \eqref{eq:points_int}. For each $y^{\ell_k}_i$, compute $\dtl_k(y^{\ell_k}_i)= \map^{\Delta_{\ell_k}}(y^{\ell_k}_i) - \map^{\Delta_{{\ell_{k-1}}}}(y^{\ell_{k}}_i)$ by solving the PDE \eqref{eq:ppde} on two successive mesh resolutions of $\Delta_{\ell_k}$ and $\Delta_{\ell_{k-1}}$ and computing the observable \eqref{eq:obsp}.  With the training data $\{y^{\ell_k}_i,\dtl_k(y^{\ell_k}_i)\}_{1 \leq i \leq N_k}$
train the neural network $\dtl^{\ast}_{k,NN} \approx \dtl_k$ and the Gaussian Process regressor $\dtl^{\ast}_{k,NN} \approx \dtl_k$, with suitable choice of the model hyperparameters. Assemble the ensemble model $\dtl^{\ast}_{k} = \alpha_{NN}\dtl^{\ast}_{k,NN} + \alpha_{GP}\dtl^{\ast}_{k,GP}$

\item [{\bf Step $3$}:] Form the machine learning model $\map^{\ast}_{ml} \approx \map^{\Delta_L}$ as
\begin{equation}
    \label{eq:ml_ext}
    \map_{ml}^{\ast}(y) = \map^{\ast}_0(y) + \sum\limits_{k=1}^k \dtl^\ast_k(y), \quad \forall y \in Y.
\end{equation}

\end{itemize}
\end{algorithm}



\subsection{Implementation}
\label{ch:implementation}
We provide here a concrete implementation of the multilevel machine learning model according to the next numerical examples.

\subsubsection{Ensemble Training for the Choice of the Models Hyperparameters} 
\label{sec:train}
According to Algorithm \ref{alg:ext_ML}, the training of the terms in (\ref{eq:ml_ext}) requires in the first place the definition of the hyperparameters of the surrogates ${\map}^\ast_{0, Mod}$ and ${\dtl}^\ast_{k, Mod}~, 1 \leq k \leq n$, where the subscript $Mod$ denotes one between Neural Network and Gaussian process models. Inspired by the work of Lye, Mishra and Ray \cite{lye2019deep}, we employ an \textit{ensemble training} procedure to this purpose. As far as the difference functions are concerned, we use the \textit{same} hyperparameters configuration for \textit{each} detail ${\dtl}^\ast_{k,Mod}$, $1\leq k\leq n$, defined by the ensemble training performed on the reference difference function 
\begin{equation}
	\dtl_{ref} = {\map}^{\Delta_1} - {\map}^{\Delta_0}.
\end{equation}
We implicitly assume that the behaviour of the maps ${\dtl}_{k}(y)$ is the same for all the resolution levels, that is not necessarily true in practice. We use $N^{ens}_{0}$ and $N^{ens}_{ref}$ samples to perform the ensemble trainings for the tuning of the hyperparameters of ${\map}^\ast_{0,Mod}$ and ${\dtl}^\ast_{ref,Mod}$, respectively. The selection of the best performing parameters configuration is dictated by the value of the approximate generalization error computed on the validation set, accounting for 10\% of the entire number of samples devoted to the ensemble procedure. Our choice of the reference difference function is motivated by the fact that at coarse levels we can generate a large number of samples at small expense resulting in larger validation sets and more reliable estimation of the true generalization error. 
\begin{enumerate}
	\item \textbf{Tuning of Neural Network Hyperparameter.} In the following numerical examples we follow the ensemble training procedure described in \cite{lye2019deep}.
	Based on the results achieved by the authors, we use the mean squared loss function ($p=2$ in (\ref{eq:lf1})) and we choose as optimization method the ADAM algorithm with learning rate $\eta=0.01$ in \textit{full batch} mode. We fix \textit{a priori} a reference architecture with prescribed number of layers and units  and perform an ensemble training for the selection of the exponent of the regularization term and regularization parameter. The exponent of the regularization term can be either $q=1$ or $q=2$. For the regularization parameters we use $\lambda = 5\cdot10^{-7}, 10^{-6}, 5\cdot10^{-6}, 10^{-5}, 5\cdot10^{-5}, 10^{-4}$. We also set the number of epoch to 10000 for all the ensemble configurations. 
	Here, each model is retrained 5 times and the initial configuration resulting in the smallest value of the prediction error on the validation set is picked.
	
	\item \textbf{Tuning of Gaussian Process Hyperparameter.} We employ similar ensemble procedure for the  choice of the GP covariance function. Here, we select one between the squared exponential (\ref{eq:SE_cov}) and the Matern kernel (\ref{eq:mat_cov}). The characteristic length $\ell$ of the kernels is defined by minimizing the log negative marginal likelihood \cite{}. In the case of Matern kernel, we also need to define the parameter $\nu$ appearing in (\ref{eq:mat_cov}). This results, overall, in four different configurations:
	\begin{itemize}
		\item Squared exponential kernel;
		\item Matern kernel with $\nu=0.5$;
		\item Matern kernel with $\nu=1.5$;
		\item Matern kernel with $\nu=2.5$.
	\end{itemize}
\end{enumerate}
As far as the selection of the coefficients $\alpha_i$ in the specification of the ensemble model is concerned, we proceed as follows. If the number of training points is sufficiently large ($N_K>500$), we exclude approximately 10\% of the samples from the training samples in order to perform a linear regression over the values predicted by the models. This usually occurs at the coarse levels, where several samples are available. On the other hand, at the fine resolutions, we use the standard average model, with $\alpha_1 = \alpha_2 = \frac{1}{2}$. 


\begin{comment}
\textbf{Assessment of Multilevel Predictive Performance.} 
Performances of the resulting multilevel schemes are assessed by evaluating the mean prediction error (\ref{mpe}) with $p=2$ on the testing set:
\begin{equation}
\label{spe}
{\varepsilon}_{ml}   := \frac{1}{N_{\mathcal{T}}}\Bigg(\sum_{y \in \mathcal{T}}^{N_{\mathcal{T}}}\big |\map^{(L)}(y) - \widehat{\map}^{(L)}(y)\big|^2 \Bigg)^\frac{1}{2}
\end{equation} 
We normalize the generalized error with respect to the $L^2$ norm of the observable.
Our objective is to estimate the performance of the multilevel model with respect to the single level one. To this end, we compute the relative mean prediction error ${\varepsilon}_{sl}$ achieved with the classical single level algorithm, trained  by using $M_{sl}$  samples at the finest resolution, with $M_{sl}$ chosen so that the computational cost required for generating the sequence of datasets $D_k$ for the multilevel scheme is equal to the cost needed to generate $M_{sl}$ samples at the finest level. As far as the learning models hyperparameters are concerned, we employ the same best performing configuration obtained for the approximate model at the coarsest resolution. We introduce the \textit{accuracy speed up}, defined as:
\begin{equation}
G = \frac{{\varepsilon}_{sl} }{{\varepsilon}_{ml} }.
\end{equation}
The accuracy efficiency represents the variable of major importance in order to assess the predictive efficiency of the multilevel scheme and it is the fundamental target of the sensitivity study to the multilevel models design parameters. However, it does not take into account the influence of the model parameters on the computational cost of the model and the overall performance of the multilevel model.  
\end{comment}

\subsubsection{Sensitivity Study to the Design Parameters}
\label{sec:sens}
The design of a multilevel scheme demands the definition of three fundamental ingredients:
\begin{itemize}
	\item The sequence $s_n = \{\ell_k\}_{k=1}^n$ of mesh resolutions that results into a specific model complexity $c_{ml}$;
	\item The number of training samples $N_0$ to learn the map $\map^{(0)}(y)$ at the coarsest resolution level;
	\item The number of training samples $N_L$ to learn the detail $\dtl^{(n)}(y) = \map^{(\ell_n)}(y) - \map^{(\ell_{n-1})}(y) $;
\end{itemize}
A sensitivity study can be performed to assess the influence of the \textit{design parameters} and  provide a guideline for the optimal design of the multilevel model.  In particular, our objective is to estimate the performance of the multilevel model with respect to the single level one. To this end, for each choice of the design parameters, we run Algorithm \ref{alg:ext_ML}  with  the model hyperparameters selected as described in Section \ref{sec:train} and we train the corresponding standard learning models $\map^\ast_{sl, NN}$ and $\map^\ast_{sl, GP}$ by using $N_L^{sl}$ samples at the resolution $\Delta_L$, chosen such that the total cost of the two competing models is the same. The same configuration of hyperparameters found to perform best for $\map^\ast_{0}$ is used for $\map^\ast_{sl}$, as well.  We build the ensemble model also for the standard scheme. Once the models training is complete, performances of the competing models are evaluated by computing the generalization error on the testing set:
\begin{equation}
\label{spe}
{\er}  := \frac{1}{N_{\test}}\Bigg(\sum_{y \in \test}^{N_{\test}}\big |\map^{\Delta_L}(y) - {\map}^\ast(y)\big|^2 \Bigg)^\frac{1}{2}.
\end{equation} 
The generalization error is normalized with respect to the $L^2$ norm of the observable.
For each configuration of the design parameters, the accuracy speed up of the multilevel model with respect to standard one can be computed as 
\begin{equation}
    G = \frac{\er_{sl}}{\er_{ml}}.
\end{equation}
The sensitivity study aims at providing the set of configurations resulting in the greatest speed up and the overall best performing ones \footnote{We refer to the accuracy speed up instead of the speed up $\frac{1}{\Sigma_{ml}}$ foe convenience of calculation}.





\subsubsection{Uncertainty Quantification}
\label{ciao} 
In context of UQ, the performance of Monte Carlo and Multilevel Monte Carlo are compared with the machine learning models, with particular focus on the novel scheme presented in this work. We are interested in the estimation of the mean value, standard deviation and probability distribution of the observable $\map$. The performances of competing schemes are assessed by comparison with a reference solution computed by using a large number of samples at fine mesh resolution. The accuracy of the estimation of the mean and the standard deviation is evaluated by computing the relative error:
\begin{equation}
e_E = \frac{\Big|\widehat{E}[\map^{(L)}] - \E{\map}_{ref}\Big|}{\Big|\E{\map}_{ref}\Big|}, \quad\quad e_\sigma = \frac{\Big|\widehat{\sigma}[\map^{(L)}] - \sigma[{\map}]_{ref}\Big|}{\Big|\sigma[{\map}]_{ref}\Big|},
\end{equation}
where $\E{\map}_{ref}$ and $\sigma[{\map}]_{ref}$ denote the mean and the variance of the observable of the reference solution. 
On the other hand, the accuracy of the probability distribution estimation is assessed by means of the Wasserstein distance $W$ \cite{opt_tran}.
For the machine learning schemes we proceed as described in Section \ref{sec:4}. The trained models are fed with $J_L=10000$ uniformly distributed samples $\{y_i\}_{i=1}^{J_L}$ and the corresponding observable values returned by the approximate models used to estimate the statistics of the observable. We compute the mean value of the relative errors by averaging the results obtained by $K=30$ independent resamplings of the data points $\{y_i\}_{i=1}^{J_L}$:
\begin{equation}
\mathcal{R}E_E = \sqrt{\frac{\sum_{k=1}^{K} e_{E,k}^2}{K}}, \quad\quad \mathcal{R}E_V= \sqrt{\frac{\sum_{k=1}^{K} e_{\sigma,k}^2}{K}}, \quad\quad \mathcal{R}E_W= \sqrt{\frac{\sum_{k=1}^{K} W_k^2}{K}}.
\end{equation}
For the statistical sampling methods we refer to \cite{} and references therein. 

\subsection{Code}
All the numerical results presented below are based on the following codes:
\begin{itemize}
    \item The data sets for the first numerical example are generated with the support of a Python solver that employs the simple \textit{first order forward-Euler} discretizazion algorithm.
    \item The data sets for the two-dimensional Euler equations are generated using TEnSUM, which is a vertex-centered finite-volume solver for compressible flows on unstructured triangular grids \cite{}.
    \item The assembling of the multilevel models and the ensemble training for the selection of the model hyperparameters  are performed with a collection of Python scripts, with the support of Keras \cite{}, Tensorflow \cite{} and Scikit-learn \cite{}.
\end{itemize}
The scripts for the generation of the data set for the first example and the construction of the multilevel model can be downloaded from \textbf{link}.

==> Old/introduction.tex <==
\section{Introduction}

==> Old/theory.tex <==
\section{Convergence theory}
